Force-feedback based Whole-body Stabilizer for Position-Controlled Humanoid Robots

This paper studies stabilizer design for position-controlled humanoid robots. Stabilizers are an essential part for position-controlled humanoids, whose primary objective is to adjust the control input sent to the robot to assist the tracking controller to better follow the planned reference trajectory. To achieve this goal, this paper develops a novel force-feedback based whole-body stabilizer that fully exploits the six-dimensional force measurement information and the whole-body dynamics to improve tracking performance. Relying on rigorous analysis of whole-body dynamics of position-controlled humanoids under unknown contact, the developed stabilizer leverages quadratic-programming based technique that allows cooperative consideration of both the center-of-mass tracking and contact force tracking. The effectiveness of the proposed stabilizer is demonstrated on the UBTECH Walker robot in the MuJoCo simulator. Simulation validations show a significant improvement in various scenarios as compared to commonly adopted stabilizers based on the zero-moment-point feedback and the linear inverted pendulum model.

==> comments/reviews.tex <==
1. The main drawback is the lack of experiments on real platforms.
2. Since the final outcome is clearly an admittance law, authors should really spend a few words on how their approach compares to such a control scheme.
3. Keep the second term in (12) if we know the actuator model.
4. To explain how a simplified model LIPM is limited in more detail giving some examples.
5. More detailed analysis is required compared to ZMP feedback
6. In Fig.4 and Fig.5, why is the moment around x-axis almost zero while that around y-axis is not so.
